Analyzing the numerical correctness of branch-and-bound decisions for mixed-integer programming

Most state-of-the-art branch-and-bound solvers for mixed-integer linear programming rely on limited-precision floating-point arithmetic and use numerical tolerances when reasoning about feasibility and optimality during their search. While the practical success of floating-point MIP solvers bears witness to their overall numerical robustness, it is well-known that numerically challenging input can lead them to produce incorrect results. Even when their final answer is correct, one critical question remains: Were the individual decisions taken during branch-and-bound justified, i.e., can they be verified in exact arithmetic? In this paper, we attempt a first such a posteriori analysis of a pure LP-based branch-and-bound solver by checking all intermediate decisions critical to the correctness of the result: accepting solutions as integer feasible, declaring the LP relaxation infeasible, and pruning subtrees as subopti mal. Our computational study in the academic MIP solver SCIP confirms the expectation that in the overwhelming majority of cases, all decisions are correct. When errors do occur on numerically challenging instances, they typically affect only a small, typically single-digit, amount of leaf nodes that would require further processing.

==> TMP_snippets.tex <==

%%%
%%% TEXT SNIPPETS TO THROW AWAY OR USE ELSEWHERE
%%%




********** OMIT OR MOVE TO PRELIMINARIES **********

pseudo-Boolean formulas are in effect just another syntactic way of writing \mbox{$0$--$1$}  integer linear programs in the form
\begin{align*}
\min
&& \sum_{j\in N} c_j & x_j\\
\text{s.t.}
&& \sum_{j\in N} a_{ij} & x_j \geq b_i && \text{for } i\in\{1,\ldots,m\} \eqcomma\\
&&& x_j \in \{0, 1\} && \text{for } j \in N = \{1,\ldots,n\} \eqcomma
%\label{eq::pseudoboolean}
\end{align*}
with all $c_{j}, a_{ij}, b_i\in\mathbb{Z}$.
%
In the interest of readability, we will drop the row index~$i$ in constraints whenever this does not create ambiguity.
%
When convenient, we refer to a pair of constraints $E_{\geq} \synteq \sum_{j\in N} a_{j} x_j \geq b$ and $E_{\leq}  \synteq \sum_{j\in N} -a_{j} x_j \geq -b$ as an \emph{equality} $E \synteq E_{\geq}  \land E_{\leq} $.
% 
As a result, MIP solvers can be applied to solve pseudo-Boolean decision and
optimization problems directly \cite{BertholdHeinzPfetsch2008}, and are quite competitive for decision problems and most often superior for optimization problems \cite{DGN21LearnToRelax,DGDNS21Cutting}.

